Cauchy transforms arising from homomorphic conditional expectations parametrize free Pick functions but those arising from conditional expectations do not

Nevanlinna showed that Cauchy transforms of probability measures parametrize all functions from the upper half plane into itself satisfying a certain asymptotic condition at infinity. We show that the correspondence fails in general for the unbounded case for somewhat trivial reasons; however, we show that in a setting of "homomorphic" operator valued free probability that Cauchy transforms of homomorphic conditional expectations parametrize free Pick functions.

==> freefunctions.tex <==

\section{Free analysis}
%
%Let $M_n(\C)$ denote the set of $n\times n$ matrices with complex entries. We define the $d$-dimensional matrix universe to be
	%$$ \mathcal{M}^d = \bigcup_{n\in \mathbb{N}} M_n(\mathbb{C})^d.$$ 
%
%A free set $\mathcal{D} \subset \M^d$ satisfies the following properties:
%
%\begin{enumerate}
%\item $A, B \in \mathcal D \Leftrightarrow A \oplus B \in \mathcal D$.
%\item $\forall A \in \mathcal{D} \cap M_n(\C)^d, \forall U \in U_n(\C), U\ad A U \in \mathcal D$.
%\end{enumerate}
%
%We define a \dfn{free function} on $\mathcal D \subset \mathcal{M}^d$ to be a function
%$f: \mathcal{D} \rightarrow \mathcal{M}^1$ which satisfies the following:
		%\begin{description}
	%\item[$f$ is graded] $X \in \mathcal{D}\cap M_n(\mathbb{\C})^d \Rightarrow f(X) \in M_n(\mathbb{C})$
	%\item[$f$ respects direct sums] 
	%$X, Y \in \mathcal{D}$ then
	%$$
	%f\left(\begin{matrix} X & \phantom 0 \\ \phantom 0 & Y \end{matrix}\right)
	%=\left(\begin{matrix} f(X) & \phantom 0 \\ \phantom 0 & f(Y) \end{matrix}\right)
	%$$
	%\item[$f$ respects similarity]
	%If $X, S^{-1} X S \in \mathcal{D}\bigcap M_n(\mathbb{C})^d, S \in GL_n(\C)$, then
	%\[
	%f(S^{-1} X S) = S^{-1} f( X )S.
	%\]
	%\end{description} 
%\red fix. \blue
%Free functions can be extended naturally to matrix-valued outputs. Say that a function $f$ is a matrix-valued free function if
	%$$f(x) = (f_{ij}(x))_{ij}$$
%where each $f_{ij}(x)$ is a free function.
%\black 
%
%Let $\Xi \subset \mathcal M^1$ be the set 
	%$$\Xi = \{X : \RE X > 0\}.$$
%A free function $h$ on a free set $\mathcal D$ is a \dfn{free Herglotz function} if $h:\mathcal D \to \Xi$.
%
%We will consider free sets consisting of block matrices. Let 
	%$$\mathcal B_n^{m\times m} = \{ X \in \tensor{M_{m}(\C)}{M_n(\C)}: \norm{X} < 1\},$$
%and let 
	%$$\mathcal B^{m\times m} = \cup_{n=1}^\infty \mathcal B_n^{m\times m} \subset \tensor{M_m(\C)}{\M},$$ 
%that is $\mathcal B^{m \times m}$ is an $m\times m$ \dfn{contractive block domain}, the set of $m \times m$ block matrix contractions with $n\times n$ matrix entries. A \dfn{free block Herglotz function} is a free Herglotz function on a block contractive domain.
%
%The following representation is proved by the authors in \cite{ppt16}. A related theorem can be found in \cite{popescumajorant}.
%\begin{proposition} \label{hergrep}
%If $h$ is a free Herglotz function on the block domain $\mathcal B^{m \times m}$, then there exist a matrix $B \in M_m(\C)$, a separable Hilbert space $\hilbert$, an isometry $V: \C^m \to \tensor{\hilbert}{\C^m}$, and a unitary $L: \tensor{\hilbert}{\C^m} \to \tensor{\hilbert}{\C^m}$ such that
	%$$h(X) = -i \tensor{B}{I} + \tensor{V\ad}{I} \left(\tensor{L}{I} - \tensor{I_\hilbert}{X} \right)\inv \left( \tensor{L}{I} + \tensor{I_\hilbert}{X}\right)\tensor{V}{I}.$$
%\end{proposition}
%
%
%Likewise, let 
	%$$\Pi^{m\times m}_n = \{ Z \in \tensor{M_m(\C)}{M_n(\C)}: \IM Z > 0\}$$
%and let 
	%$$\Pi^{m\times m} = \cup_{n=1}^{\infty} \Pi^{m\times m}_n \subset \tensor{M_m(\C)}{\M}.$$
%The set $\Pi^{m\times m}$ is the \dfn{block upperhalfplane}. A \dfn{free block Pick function} is a free function $f: \Pi^{m\times m} \to \Pi$. 
	%
%\red 
%A free Herglotz funciton is a free function $h: \Ball{B_1} \to \RHP{B_2}$.
	%
	%
%The Cayley transform 
	%$$ z = i \frac{1 + x}{1 - x}, \hspace{.2in} x  = \frac{z - i}{z + i}$$
%provides a one-to-one correspondence between $\B^{m\times m}$ and $\Pi^{m\times m}$. Work of G. Popescu extends the Cayley transform in the free setting to relate conformally equivalent classes of free functions \cite{po08}.
